On the Threat of npm Vulnerable Dependencies in Node.js Applications

Software vulnerabilities have a large negative impact on the software systems that we depend on daily. Reports on software vulnerabilities always paint a grim picture, with some reports showing that 83% of organizations depend on vulnerable software. However, our experience leads us to believe that, in the grand scheme of things, these software vulnerabilities may have less impact than what is reported. Therefore, we perform a study to better understand the threat of npm vulnerable packages used in Node.js applications. We define three threat levels for vulnerabilities in packages, based on their lifecycle, where a package vulnerability is assigned a low threat level if it was hidden or still unknown at the time it was used in the dependent application (t), medium threat level if the vulnerability was reported but not yet published at t, and high if it was publicly announced at t. Then, we perform an empirical study involving 6,673 real-world, active, and mature open source Node.js applications. Our findings show that although 67.93% of the examined applications depend on at least one vulnerable package, 94.91% of the vulnerable packages in those affected applications are classified as having low threat. Moreover, we find that in the case of vulnerable packages classified as having high threat, it is the application's lack of updating that makes them vulnerable, i.e., it is not the existence of the vulnerability that is the real problem. Furthermore, we verify our findings at different stages of the application's lifetime and find that our findings still hold. Our study argues that when it comes to software vulnerabilities, things may not be as bad as they seem and that considering vulnerability threat is key.

==> npm Vulnerability Threats/background.tex <==
%This section provides a brief overview of vulnerabilities terminologies and other terminologies  in general. 
%Also, we explain how we collect and prepare the data for our research questions.

% dependencies handling in Node.js application example cartodb applications, active
%\subsection{Terminology}
%\emad{Need to have a formal definition and provide a citation for the definition of a vulnerability.}
%A software vulnerability is a weakness that allows performing unauthorized actions and/or allow unauthorized access to a given software system~\cite{liu2012software}.
%When software developers find a vulnerability in packages they maintain, they generally report and fix the vulnerability and after that, they notify CVE Numbering Authority (CNA), which is an organization that can assign and announce Common Vulnerability Exposure (CVE) entries, to assign a CVE identifier (CVE ID) to the vulnerability. This comprises CVE databases, and when developers become aware of such case, they can fix it, e.g., by using newer versions. \emad{I think that a vulnerability can also be found by users. We need to explain that path.}

%\emad{we need to have a clear diagram (maybe a state flow diagram) of the different stages of a vulnerability and who knows about it.}

In this section, we explain the different stages a vulnerability goes through in its lifecycle. Then, we define our threat levels for vulnerabilities using the different stages that a vulnerability goes through during its lifecycle.

\subsection{Vulnerability  Lifecycle}
\label{sec:background2}
A software \emph{vulnerability} is a weakness that allows unauthorized actions and/or access to be performed. These actions are typically used to break through the system and violate its security policies~\cite{liu2012software,shirey2000internet}. A \emph{vulnerability threat} is a 
potential danger to exploit a vulnerability in order to breach security and cause possible harm~\cite{shirey2000internet}.
%``possible danger that might exploit a vulnerability to breach security and therefore cause possible harm''~\cite{shirey2000internet} \emad{Mahmoud, make sure it is consistent with the def in the intro}. 
As shown in Figure~\ref{vuln_timeline}, typically, and with emphasis on vulnerabilities in the Node Package Manager (\npm ecosystem), a vulnerability goes through a number of different stages~\cite{Reporting96}.

\begin{itemize}
\item \textbf{Introduction.} This is when the software vulnerability is first introduced into the code. At this stage, no one really knows about its existence, assuming that the introduction is not malicious. Hence, the potential threat of the vulnerability is quite low. 

\item \textbf{Discovery (report).} When a vulnerability is discovered, it must be reported to the npm security team. The npm team investigates to ensure that the reported vulnerability is legitimate. At this stage, only the security team and the reporter of the vulnerability know about its existence. The  potential threat at this stage is still low.
 %that can damage the system at this point is higher than the previous stage since some vulnerability information get discovered (uncovered in private).
%
\item \textbf{Notification.} Once the reported vulnerability is confirmed, the security team triages the vulnerability and notifies the vulnerable package maintainers. At this stage, only the reporter, npm team, and package maintainers know about the vulnerability, hence its potential threat to be exploited remains low.

%existence. However, package maintainers also know about the vulnerability existence at this stage. The potential threat at this point is very close to the \textit{Discovery stage} because package maintainers are now informed about the vulnerability and should have started working on the fix.
%
%
\item \textbf{Publication without a known fix.} Once the package maintainers are notified, they have 45 days before npm publishes the vulnerability publicly. 
Alongside with publishing the vulnerability, the npm team may also publish a proof-of-concept showing how the vulnerability can be exploited. 
At this stage, the vulnerability is known publicly and its potential threat is high.

\item \textbf{Publication with a fix.} Another (and more common) way that a vulnerability can be published is when a fix is provided by the package maintainers. If a fix is provided (before 45 days), then npm publishes the vulnerability along with the version of the package that fixes the vulnerability. At this stage, the potential threat is not as high as when a no fix is provided, but now the onus is on the application maintainers to make sure that they pull in the latest fixes, otherwise they are risking being exploited.
\end{itemize}

Typically, the vulnerability publish date is after the report and notification dates. It is important to note that although the aforementioned stages are generally sequential, we do see cases where {it is not}. For example, in some cases we see vulnerabilities with a fix date that precedes its reporting or publication
date. The race between developers and attackers starts as soon as a vulnerability is discovered. We use the different stages of a vulnerability to examine the potential threat of software vulnerabilities next.

\subsection{Threat Levels}
\label{sec:ex}

As shown earlier, the different stages that a vulnerability goes through significantly impact its threat. Hence, our study is based on the idea that vulnerabilities should be examined while taking their threat into consideration as the \textit{vulnerability timing} makes them hard to exploit. We use the various stages to ground our argument and define three specific threat levels:

\begin{enumerate}

\item \textbf{Low threat - before discovery (report).} Since very little (or nothing at all) is known about a vulnerability before it is found, i.e., vulnerabilities are hidden in the applications, we believe that its potential threats and chances of being exploited are very low. Hence, we classify all vulnerabilities at this stage as having \emph{low threat}.

\item \textbf{Medium threat - after discovery \& before publication:} Once a vulnerability has been discovered, there is potential that others may also know about it. Moreover, since at this stage the public is still not aware of the vulnerability, 
%and the proof-of-concept of its exploit may not be published,
the vulnerability might be exploited by people who know about it somehow and have the capability to exploit it. Hence, we classify vulnerabilities at this stage as having \emph{medium threat}.

\item \textbf{High threat - after publication:} After publication %and because the proof-of-concept is published, 
this is the time when the chance of exploitability is highest. Of course, if a fix is provided, then the risk is lower, however, if the application does not update then it still faces a major risk of  being exploited. If a fix is not provided, then all applications are at a very high risk of being exploited, hence, we classify all vulnerabilities at this stage as having \emph{high threat}.
\end{enumerate}




%The life-cycle of a vulnerability goes through different stages as we explained earlier in Section 2.1,  and so does the risk they bring to the depending applications.
%
%Many vulnerability scanners \footnote{http://retirejs.github.io/retire.js/} \footnote{https://snyk.io/} \footnote{https://gemnasium.com/} track multiple resources like bug reports and mailing lists in addition to vulnerability databases and notify the software maintainers about reports related to their dependencies.
%
%The essential idea behind this type of tools is to notify the developers, as soon as possible, about vulnerability reports related to their dependencies once they are available.
%Because once the vulnerability is discovered or publicly announced, it is a race on between developers and hackers to fix or exploit the vulnerability.
%
%From this point of view we notice that when assessing the risk of a vulnerable dependency, it is essential to take into consideration the temporal position of the analysed snapshot of the application in comparison with the introduction, discovery, and publication times. \\
%This kind of risk assessment is orthogonal and complementary to the risk assessment of vulnerabilities used in vulnerability reports. 
%
%To get a clear picture of the temporal risk assessment, let us consider the following cases which illustrate the increase in risk based on the temporal position of the application Snapshot Time (ST) and taking into consideration the users' awareness of the vulnerability existence as described in Section 2.1.
%%as seen in Figure~\ref{vuln_timeline}:
%\begin{itemize}
%	\item If the application at ST was relying on vulnerable version of the dependency D, and the vulnerability that affects the version was not {reported} yet at that time, then the threat it imposes on the application is lower that what it would be if the vulnerability gets discovered.
%	\textit{(ST $\leq$ vulnerability discovery time).}
%	We classify the application in this case: \textit{\textbf{low exploitability} level}
%	
%	\item If the application at ST was relying on a vulnerable version and the vulnerability that affects the version was reported to the npm Security team but not yet published, then the threat it imposes on the application would be more than the previous category, but still not as risky as the next one.
%	\textit{(vulnerability report time $\leq$ ST $<$ vulnerability publication time).}
%	We classify the application in this case: \textit{\textbf{medium exploitability} level}
%	
%	\item If the application at ST was relying on vulnerable version of the dependency D, and the vulnerability was published, then the threat it imposes on the application is the highest.
%	\textit{(ST $>$ vulnerability publication time).}
%	We classify the application in this case: \textit{\textbf{high exploitability} level}
%	
%\end{itemize}
%\emad{we need to re-write this and simplify it so that we convince people of our defined levels. Right now, it feels like we wrote it to tell them what our levels are.}
%
%The life-cycle of a vulnerability goes through different stages~\cite{frei2010modeling}:
%the vulnerability introduction, disclosure, and publication time. Based on that, we introduce the \textit{levels of exploitability} of the vulnerable dependency which captures the temporal position of the analysed snapshot of the application in comparison with the introduction, disclosure, and publication time,
%i.e., if an application relies on a dependency that is vulnerable but whose vulnerability report has not yet been disclosed or published, then the vulnerability will have a lower chance of being exploitable, hence the attribute \textit{low exploitable}.

% a vulnerable dependency according to when an application's snapshot/release is taken to be scanned for vulnerabilities, i.e., if an application relies on a vulnerable dependency that its vulnerability report has not been yet disclosed or published, it is actually not exploitable, and hence, we consider the vulnerability of such dependency as "low exploitable".
%
%To clearly understand the levels of exploitability, let us assume we have an application A and we would like to assess the dependencies of this application against  security vulnerabilities at a specific release or snapshot of the application, e.g., we take latest snapshot (LS) of the application and we want to assess the dependencies that existed at that snapshot against security vulnerabilities. Assume that the application (at LS time) was  relying on version one of dependency D which is affected by a vulnerability.
%
%Now, to measure the exploitability level of this vulnerability that affects version V of dependency D in the application, we compare the time in which the snapshot of the application was taken (i.e., LS time) with the different stages of the vulnerability lifetime, i.e.,  vulnerability introduction time, vulnerability disclosure time, and vulnerability publication time. Based on that, we come up with the following exploitability levels as shown in Figure~\ref{vuln_timeline}:

%Figure~\ref{vuln_timeline} illustrates two timelines. The above one presents the vulnerability timeline of version one of the dependency D, assuming that this version is vulnerable. The below timeline presents the application timeline. 
%Let us assume that the application was relying on
%dependency D at release four (r4 snapshot) of the application. Also, we assume that version one was the latest installable and satisfying version of dependency D at the time of r4.

\begin{figure}[tb!]
	\centering
	\includegraphics[width=1\linewidth]{images/vuln_timeline_new}
	\caption[]{Classification of threats over the vulnerability lifecycle.} %\emad{Mahmoud, remove the word Vulnerability in the Fig}.}
	%\setlength{\abovecaptionskip}{40pt}
	\label{vuln_timeline}
\end{figure}

%So, the million dollar question is "what was the exploitability level of version 1 of dependency D when r4 snapshot of the application is taken?"
%In this context, we introduce three levels of exploiting a vulnerable dependency in the application. The exploitability levels are as follows:
%\begin{itemize}
%	\item \textbf{low exploitability}: we consider the vulnerable dependency found at the time in which we scan for vulnerable dependencies (i.e., LS time) as low exploitable \textit{IF LS time is equal or less than the vulnerability disclosure time (LS $\leq$ vulnerability disclosure time)}, i.e., the application was relying on a vulnerable version of the dependency at LS time and the vulnerability was not disclosed at that time, and hence, it is less likely to create a threat to exploit it which makes the application less exploitable.
%%
%	 %the snapshot time in which we scan for vulnerabilities and the application was depending on the vulnerable dependency is \textit{before} the vulnerability becomes disclosed, we consider the exploitability level of the vulnerability that affects the dependency in the application as \textbf{low exploitability}. 
%	%we consider the level of exploitability as low if the time of installing a vulnerable version of a dependency was before the vulnerability has been disclosed, i.e.,\\
%	%vulnerability introduced  $\leq$ r4 $<$ vulnerability disclosed. 
%	\item \textbf{medium exploitability}: we consider the vulnerable dependency found at the time in which we scan for vulnerable dependencies (i.e., LS time) as medium exploitable \textit{IF LS time is greater than the vulnerability disclosure time AND LS is equal or less than the vulnerability publication time.
%	(vulnerability disclosure time $\leq$ LS $<$ vulnerability publication time)}, i.e., the application was relying on a vulnerable version of the dependency at LS time and the vulnerability was disclosed but not yet published at that time, and hence, the application is of medium exploitability.
%
%	\item \textbf{high exploitability}: we consider the vulnerable dependency found at the time in which we scan for vulnerable dependencies (i.e., LS time) as highly exploitable \textit{IF LS time is greater than the vulnerability publication time (LS $>$ vulnerability publication time)}, i.e., the application was relying on a vulnerable version of the dependency at LS time and the vulnerability was disclosed and published at that time, and hence, the application is of high exploitability.
%\end{itemize}

%\emad{we should try to avoid presenting data and leave that to Section3. However, I think we need to introduce the notion of a package vs. application and say that we are focusing on vulnerabilities in packages/dependencies. We should also have a convincing reason as to why we focus on vulnerabilities in dependencies - do we have a reason?}
%We examine our collected 11,288 applications to study to which degree those applications depend on vulnerable dependencies generally, and for each vulnerable dependency used in each application we analyse to which degree such vulnerable dependencies are exploitable based on the levels of exploitability we introduced earlier. The application may depend on more than one vulnerable dependency, and the vulnerable dependencies may be of different exploitability levels. Hence, we need a mean to decide about the exploitability level of the whole application. In our analyses, we decide the exploitability level of the application based on the \textit{weakest link}, i.e., we consider the application of low exploitability if it depends on vulnerable dependencies of low exploitability only. If the application depends on at least one vulnerable dependencies of medium dependencies,  (it could depend on low level but being the high level absent), we consider the application as of medium exploitability. Lastly, if the applications depends on at least one vulnerable dependency of high exploitability level (it could depend on low and medium ones as well), we consider the application as highly exploitable. 
%
%At first, we conduct the exploitability level analysis over the latest snapshot of the applications.
%Later on, we conduct the same analysis, however, we consider the historical view of the applications development timespan, i.e., we consider different historical snapshots of each application.

%%The \textit{npm} package manager provides metadata for each library, e.g.,
%name, versions, dependencies, and dependants. The dependencies of a library are
%the libraries (name and version) that it requires to function, while the library's dependants are the libraries for which it is a dependency itself. %  is  by a package to execute packages by another package or application who depends on these dependencies.
%For each dependency, a package also specifies a constraint. Such
%a dependency constraint uses \textit{semantic versioning}, a practice to assign meaningful
%version numbers to a dependency. % It is used to specify the
%% allowed versions of dependencies. 
%For example, a dependency constraint
%can specify the maximum allowed version (e.g., <=1.1.2) or
%the minimum version (e.g., >=3.2.1). However, a combination of both
%minimum and maximum can be
%specified as well, by using other types of constraints involving special operators (\textasciicircum, \textasciitilde).
%The == operator is used for an exact version number, while the start * operator is used to accept any version number of the dependency.
% TODO
% More details about the meaning of the remaining constraints in \textit{semantic versioning} are available online\footnote{https://docs.npmjs.com/about-semantic-versioning}.
%\bram{discuss background of (major.minor.patch) versioning}

% vulnerabilites handling
% We also would like to briefly explain how vulnerabilities are handled.

% In this study, we call an application who includes vulnerable dependency as a vulnerable application.
% CNA gives a CVE ID for the vulnerability. CVE
% databases\footnote{https://cve.mitre.org/} (which store vulnerability information using CVE
% ID as a key) and security information providers (which store
% vulnerability information with or without CVE ID), enter the
% vulnerability information to their databases. If someone notices the vulnerability
% information from these databases, and he/she knows that another
% application is affected by the vulnerability, they report it to the application. 
% We call an application as affected
% application. The developers of affected applications handle the reported vulnerability (e.g., by using fixed versions).



==> npm Vulnerability Threats/conclusion.tex <==
Our study examined software vulnerabilities in npm dependencies with respect to their threat on the dependent Node.js applications. First, we defined three levels of threat for software vulnerabilities in dependencies based on their lifecycle and performed an empirical study on 6,673 Node.js applications to assess how threatening the vulnerable dependencies that exist in these applications really are. Our findings indicate that the vast majority of vulnerable dependencies have low threat on applications that depend upon them. 
Although 67.93\% of the examined applications depend on at least one vulnerable package, 94.91\% of the vulnerable dependencies are classified as having low threat.
Moreover, we examined why these applications end up depending on high threat vulnerable versions of these dependencies. We observed that, in the case of high threat vulnerabilities, the applications are to blame in more than 87\% of the cases, i.e., a fix for the vulnerable dependency is available but not patched in the application.
These findings show that the assumption that all vulnerabilities that exist in packages will impact applications the same way is not correct and that vulnerable packages are not always to blame. Finally, our further analysis shows that all of the observed trends hold across the different stages of the applications' lifetime.

In the future, we plan to further elaborate on the impact of the various threat vulnerabilities on the applications' functionality level. Other data sources  can be added to enhance the risk assessment, e.g., severity, exploitability, etc.  We also aim to examine if our findings hold for applications written in different programming languages.

==> npm Vulnerability Threats/dependency.tex <==
%\diego{Improve this beginning. It seems only loosely connected.}
We use our defined threat levels to examine vulnerable dependencies in Node.js applications. Since determining vulnerable dependencies heavily relies on the management of the dependencies and how they are resolved, in this section, we highlight how npm dependency management works.

Node Packages Manager (npm) is the main package manager used by Node.js applications to manage their dependencies~\cite{npmregis47:online}. npm has a registry where packages are published and maintained.
To date, npm registry hosts more than 1.3M packages, and has had the highest growth rate in terms of packages amongst all known programming languages~\cite{npmLibra8}.
%\emad{according to libraries.io it is more than 1.3M}

To determine the threat of vulnerable dependencies in Node.js applications, we need to 
understand two important mechanisms of the npm ecosystem: 1) how Node.js applications specify their npm dependencies and 2) how npm resolves a dependency version, i.e., find the dependency version to install in a Node.js application.
Node.js applications specify their dependencies in a JSON-format file, called package.json, which lists the dependencies and their versioning constraints. The versioning constraint is a convention to specify the dependency version(s) of the package that an application is willing to depend upon.
The version constraints can be static, requiring a specific version of the dependency (e.g., ``P:1.0.0'' ), or dynamic specifying a range of versions of the dependency (e.g., ``P:$>$1.0.0''). Typically, developers use dynamic versioning constraints if they want to install the latest version of a dependency, allowing them to get the latest updates/security fixes of the package. When a dynamic version is used, the resolved version (i.e., the actual version) corresponds to the latest installable version that satisfies the constraint~\cite{cogo2019empirical}.

%In the following paragraphs, we describe both mechanisms in detail.
%how Node.js applications specify their npm dependencies. Furthermore, we need to understand how to resolve a dependency version, i.e., find the actual installed version of the vulnerable dependencies in a Node.js application. Therefore, this section provides such understanding of how npm selects the actual package version to be installed by the dependent Node.js application.


%\diego{Do we really need to define this?}
%npm adopts a semantic version numbering scheme~\cite{Semantic}. In this scheme, the version number has three figures in the format of MAJOR.MINOR.PATCH (e.g., ``1.0.0'' in the above example). An increase in the PATCH number indicates bug fixes, an increase in the MINOR number indicates additions or changes that are backwards compatible, and an increase in the MAJOR number indicates breaking changes.
%npm also adopts a grammar that is used for specifying dynamic versioning constraints. The grammar consists of a set of operators: e.g., the tilde operator (``P:\textasciitilde $1.0.0$'') matches the most recent PATCH version of the package, the caret (\textasciicircum) operator matches the most recent MINOR version, and the wild-card operator (*) allows getting the latest version of the package. The complete set of grammars for defining dynamic cab be found at~\cite{semvernp91}. In our study, we utilize a tool called, \textit{semver} to resolve the dependency versioning constraint that is defined by the application.

%\diego{Too verbose.}
Node.js applications can specify two sets of dependencies in their package.json file: development and production dependencies. Development dependencies are installed only on development environments, and consequently, issues that may arise from them (e.g., vulnerabilities and bugs) have no impact on production environments. On the other hand, production dependencies (also called runtime dependencies) are installed on both production and development environments. In our work, we only consider production %\emad{We never use the term runtime before, we use development and production. We should use production instead I believe.} 
dependencies in our analysis since they are the ones that impact the production environment~\cite{decan2018empirical}.

%\begin{figure}[htp!]
%  \centering
%  \includegraphics[width=1\linewidth]{images/npmByyears.pdf}
%  \caption[]{Growth in ecosystems.~\cite{Moduleco64:online}}
%  \label{npm}
%\end{figure}

==> npm Vulnerability Threats/design.tex <==
To examine the degree to which applications rely on vulnerable dependencies and how threatening such vulnerable dependencies are within the applications, we study a large dataset of mature and active Node.js applications that use external dependencies.
First, we describe our data collection in Section~\ref{subsec:data}.
Then, in Section~\ref{subsec:scanning} we explain how we use our threat levels to identify and classify the vulnerable dependencies in the Node.js applications. We leverage the collected data to answer the following research questions.
\begin{itemize}
	\item  \rqone 
	\item  \rqtwo 
	\item  \rqthree
\end{itemize}

\subsection{Data Collection}
\label{subsec:data}

% dataset of applications and dataset of vulnerabilities.
Our study examines vulnerable dependencies in Node.js applications. We chose to focus on Javascript due to its wide popularity amongst the development community~\cite{StackOve70:online}. % which has led to a large ecosystem of  packages available via npm.
\\
%\emad{\textcolor{blue}{I think we can cite the StackOverflow report - which showed JS is no. "1" most popular}} and the prevalence of affected application by vulnerable dependencies. 

%JS is a client- and server-side programming language that has grown in popularity, especially in the last decade.
% . Recently, it has been very popular and still growing up
%Node.js is a JavaScript run-time environment, with an active research and development community~\cite{bogart2016break, wittern2016look}. 

\noindent\textbf{Packages vs. Applications.} The software community classifies JavaScript projects into two categories:
\textit{1) packages}, also referred to as libraries, which are included in other applications using dependency management tools to help facilitate and speed up development. 
Packages are referred to as "dependencies" of an application. 
\textit{2) applications} are standalone software projects, which are distinct from libraries, where they are not distributed via a package manager and are typically applications for clients and end users rather than components to build upon.
As mentioned before, the Node.js applications mainly state the packages they depend on (i.e., dependencies) in a file called package.json. 

To perform our study, we leverage two datasets: (1) Node.js applications that use {npm} to manage their dependencies, and (2) Security vulnerabilities that affect npm packages. To do so, we \textbf{(i)} obtain the Node.js applications from GitHub, \textbf{(ii)} extract their dependencies, and \textbf{(iii)} obtain the security vulnerabilities for npm packages from {npm} advisories~\cite{npmadvisories}. The dataset collection took place during May and June of 2019.\\

\noindent\textbf{(i) Applications Dataset.} To analyse a large number of open source JavaScript applications that depend on npm packages and obtain insights on their security vulnerabilities, we mine the GHTorrent dataset~\cite{GHtorrent} and extract information about all Node.js applications hosted on GitHub. The GHTorrent dataset contains a total of 7,863,361 JavaScript projects hosted on GitHub, of which 2,289,130 use npm as their package management platform (i.e., these projects contain a file called package.json). Moreover, since both Node.js \textit{packages} and \textit{applications} can use GitHub as their development repository, and our applications dataset should only contain Node.js \emph{applications}, we filter out the GitHub projects  % () some npm packages use GitHub as their development repository, we make sure that our dataset indeed only contains Node.js applications, i.e., we exclude from our list of GitHub projects 
that are actually npm \emph{packages} by checking their GitHub URL on the {{npm}} registry. The main reason that we focused on applications and not packages is because packages become exploitable only when used and deployed in an application, i.e., packages do not reside on their own in production, they should be part of applications that make use of them. This filtering excludes 328,343 projects from our list of GitHub projects as they are identified as packages and not applications.% and we exclude them from our dataset

As shown in previous studies~\cite{kalliamvakou2014promises,kula2018developers}, some projects on GitHub are immature, hence, to make this study more reliable we refined the dataset using additional filtering criteria to eliminate such immature projects. In particular, we gather applications that satisfy all the following criteria:

%
%Furthermore, to test the impact of vulnerable dependencies on end-user
% applications that depend on them, we make ensure that our dataset indeed only contains Node.js applications, i.e., we exclude GitHub projects that are actually hosted on npm platform as libraries; we check if the GitHub URL of a GitHub repository exists on the \textit{\textit{npm}} registry. If so, we exclude this repository from our dataset 
 %The command \textbf{npm view <library name> repository.url} helps us to achieve this task. This command returns the GitHub repository url of an npm library, if it exists.

%Also, to make sure that an application uses \textit{\textit{\textit{npm}}} dependency management platform, we check, for each application repository, that it includes a file called 'package.json', which specifies runtime dependencies used by the application.

%Finally, to make this study more reliable, % and to test the impact from a quality set of real-world applications, 
%, we applied the following criteria:
\begin{itemize}
\item Non-forked applications, as we do not want to have duplicated project history to bias our analysis.

\item Applications that depend upon more than two dependencies.

\item Applications that have at least 100 commits by more than two contributors, which indicates a minimal level of commit activity.

\item Applications that have had their creation date (first commit) before January 1st 2017.
Since vulnerabilities take on median 3 years to be discovered~\cite{decan2018impact}, applications in our dataset need to have a development history long enough to have had a chance for their vulnerabilities to be discovered.

%we select this criteria because applications that have had their creation date after January 1st 2017 didn't have enough lifespan to analyze their vulnerable dependencies, given the long life-cycle for vulnerability discovery~\cite{decan2018impact},%\mhmd{@Diego, Can you please check if this is OK?}
\item Applications that have had their latest commit after January 1st 2017, as we want to analyze applications that had some level of development in the last 3 years. %\diego{This will be a source of complaints, how many applications were removed with this criteria?}


%\item %\diego{Remove young projects - explain that we need to analyze projects that have at least X years of development, given the vulnerability life-cycle.} \mhmd{Do we still need this?}
\end{itemize}

After applying these refinement criteria, we end up with 6,673 Node.js applications that make use of npm packages. Table~\ref{statsApplications} shows descriptive statistics on the selected Node.js applications in our dataset. Overall, the applications in our dataset
have a rich development history (a median of 213 commits made by 4 developers and 1,657
days of development lifespan) and make ample use of external
dependencies (a median of 11 dependencies).\\



%\emad{\textcolor{blue}{begin move}}
%Second, the \textbf{applications dataset:} this dataset contains information extracted from dependency files.
%Applications list their dependencies and other information in dependency files.
%%A dependency file stores the dependency information of the application, 
%In the case of JavaScript applications, the file is called \textit{package.json}.

\noindent\textbf{(ii) Application Dependencies.}
After obtaining the applications dataset, we want to extract the history of dependency changes of all applications.
This is necessary to identify the exact dependency versions that would be installed by the application at any specific point-in-time.
As mentioned in Section~\ref{sec:dependency}, Node.js applications specify their dependencies in the package.json file, which contains %information on the project (e.g., list of contributors) and 
the dependency list, containing the dependent upon packages and their respective version constraints.
Hence, we extract all changes that touched the package.json file and associate each commit hash and commit date to their respective package.json dependency list, creating a history of dependency changes for all applications.
Note that these dependencies are not yet resolved, that is, we only have the version constraints (not the versions) for the dependencies of each application.
\\


%As mentioned above, JavaScript applications specify their dependency information in the package.json file, which contains the application's name, version, contributors' list, development and production dependencies, and license type. Hence, in order to understand the history of dependency changes of an application, we use git commands to extract all changes that touch the package.json file over the history of each application in our dataset. Then, we parse the dependency list in the package.json and extract the commit hash, commit date, dependencies list and their versioning constraints over the history of each application.
%\mhmd{revisit}
%Since the package.json may contain dependencies that are never used in the application source-code, which should be excluded when preparing the dependency data, we use \textbf{depcheck} tool~\cite{depcheck7} that helps identifying the actual dependencies used in JavaScript source code, and hence, we exclude dependencies that are defined in the package.json file but never used in the source code.
%To resolve our history of dependency changes to the actual dependency versions that would be installed at a specific point in time, we utilize the \textit{semver} tool~\cite{semvernp91}. 
%%To determine the resolved version of each dependency, i.e., to indicate which version of a referenced dependency should be installed at a specific point in time, we utilize the \textit{semver} tool~\cite{semvernp91}. 
%Semver tool is used by npm to identify the satisfying versions of a dependency.
%The tool can be used 
%
%
% and we use it to resolve the versioning constraints defined for each dependency of all applications in our dataset.
%\diego{There was something about the scheme here that I will move back if I see it has influence on the remainder of the paper.}
%
%resolves the versioning constraint that is defined by the application for each dependency, since this is the tool used by the npm to identify the satisfying versions of a dependency versioning constraint according to the adopted scheme (described in Section~\ref{sec:dependency}).

\begin{table}[tb!] 
	\centering 
	\caption{Statistics of the 6,673  studied Node.js applications. %\diego{We should add more meaningful metrics like the age of these projects, stars, number of developers...}
	}
	\label{statsApplications}
	\begin{tabular}{l|r|r|r|r}
		\toprule
		\textbf{Metric} & \textbf{Min.} & \textbf{Median($\bar{x}$)} & \textbf{Mean($\mu$)} & \textbf{Max.} \\ \midrule
		\textbf{Commits} & 100 & 213 & 384.60 & 53,872 \\
		\textbf{Dependencies} & 3 & 11 & 14.93 & 114 \\
		\textbf{Developers} & 3 & 4 & 5.33 & 52 \\
		\textbf{Lifespan (in days)} & 151 & 1,657 & 1,730.07 & 3,575 \\
		%\textbf{Watchers} & 1 & 5 & 19.85 & 2,451 \\
		%\textbf{Stars} & 1 & 6 & 210.52 & 48,765 \\
		\bottomrule
	\end{tabular}
\end{table}


\noindent\textbf{(iii) NPM Advisories Dataset.} 
To identify Node.js applications that depend on vulnerable packages, we need to collect information on npm vulnerable packages. We resort to the \textit{NPM advisories} registry to obtain the required information about all npm vulnerable packages~\cite{npmadvisories}.
The npm advisories dataset is the official registry for npm vulnerability reports, which contains a number of JavaScript vulnerabilities, specific to the Node.js-platform packages.



%In total, we collect 654 vulnerability reports on npm packages.
This dataset provides several kinds of information about vulnerable packages relevant to our study.
Each report has the affected package name, the package versions affected by the vulnerability, and the versions in which the vulnerabiliy was fixed (safe versions). %earliest package version with the vulnerability fix.%, a remediation version (i.e., versions that contain the vulnerability fix).%patches range of the vulnerable packages (helps to identify the affected and unaffected versions of the vulnerable package), 
The report also contains both the vulnerability discovered (reported) time and published time, which we use in our approach for identifying and classifying vulnerabilities (Section~\ref{subsec:scanning}).
%indicating when the vulnerability was discovered, and the vulnerability publication time indicating when the vulnerability was publicly announced, which we use in our approach for identifying and classifying vulnerabilities (Section~\ref{subsec:scanning}).
Note that a vulnerable package could be affected by several vulnerabilities (i.e., a vulnerable package appears with different vulnerability reports due to different vulnerability types).
% , and severity (H=high, M=medium, L=low).
%To gather this information, we crawled the \textit{npm} registry in November 2018 (we repeated this in February).
% To our knowledge, the vulnerability dataset is not previously available publicly, so we make it in the form of organized and structured csv file.
% We obtained all the vulnerabilities that were available on the time of collection, i.e. 2018-November.
%We repeated this process after a month and found 9 additional vulnerabilities have been added% (e.g., only nine new vulnerabilities on 2018-December)
%For each crawled vulnerability, we obtained all the aforementioned information that interest our study.

Our initial dataset contains 654 security reports that cover 601 vulnerable packages. Following the criteria filtration process applied by Decan et al.~\cite{decan2018impact},  we removed 12 vulnerable packages of the type "Malicious Package", because they do not actually introduce vulnerable code. These vulnerabilities are packages with names close to popular packages (a.k.a. typo-squatting) in an attempt to deceive users at installing harmful packages. The 12 vulnerable packages account for 12 vulnerability reports. At the end of this filtering process, we are left with 642 security vulnerabilities reports affecting 589 distinct vulnerable packages. 
These packages have combined 26,462 distinct package versions of which 13,868 are affected by vulnerabilities from our report. 
Table~\ref{dataset} shows the summary statistics for vulnerability reports on npm packages.
 
\begin{table}[tb!]
	\centering
	\caption{Descriptive statistics on the npm advisories dataset.}
	\label{dataset}
	\begin{tabular}{l|r}
		\toprule
          Vulnerability reports & 642 \\
		Vulnerable packages & 589  \\
		Versions of vulnerable packages & 26,462    \\
		Affected versions by vulnerability & 13,868 \\ 
		\bottomrule
	\end{tabular}%
	\vspace{-2mm}
\end{table}

%\begin{table}[!h]
%	\centering
%	\caption{Descriptive statistics on npm dataset}
%	\label{dataset}
%	\begin{tabular}{l|l}
%		\toprule
%		npm packages   & 910,097       \\ 
%		Versions of npm packages   & 5,202,099         \\  \hline
%		Security reports on npm & 654                 \\
%		Corresponding vulnerable packages & 601  \\
%		Versions of vulnerable packages & 26,461    \\
%		Affected versions by vulnerability & 13,868 \\ 
%		\bottomrule
%	\end{tabular}%
%	\vspace{-2mm}
%\end{table}
\begin{figure*}[tb!]
	\centering
	\setlength{\abovecaptionskip}{5pt}
	\includegraphics[width=0.7\linewidth]{images/approach.pdf}
	\caption[]{Approach for identifying and classifying vulnerable dependencies in Node.js applications.}

	\label{classifyApproach}
\end{figure*}

\subsection{Identifying and Classifying Vulnerable Dependencies in Node.js Applications}
\label{subsec:scanning}
%\mhmd{@Diego: Can you please check this section?}
To classify the threat level of vulnerable dependencies at a specific point in the development history of a Node.js application, which we refer to as the \textit{analyzed snapshot time}, we leverage 3-step approach. Figure~\ref{classifyApproach} provides an overview of our approach, which we detail below:

%To identify the vulnerable dependencies at a specific point in the history  
%of our Node.js applications and classify them across our threat levels, we provide an approach that goes into three main steps. These steps can be applied at a specific point in time taken from the examined applications. We represent this point in time as a committed version of the dependency file (package.json) in the examined application.
%From now on, we refer to the point in time at which we analyse vulnerable dependencies in the application as  ``the analysed snapshot time''.
%Figure~\ref{classifyApproach} depicts the approach that we use to identify and classify vulnerable dependencies in Node.js applications. The details of the approach can be summarized in the following steps:
%-------start old

%-------end old


%extract and resolve dependencies 
\noindent
{\textbf{Step 1. Extract dependencies and resolve versions.}}
The goal of this step is to extract applications dependencies and find the actual dependency version installed at the analyzed snapshot time.
For each application, we extract the dependency list (with the versioning constraints) at that snapshot time from the history of dependency changes.
After that, to find the actual version of each dependency at the analyzed snapshot,  we utilize the \textit{semver} tool~\cite{semvernp91} that is used by npm to find the latest version that satisfies the versioning constraint, with an additional restriction that the satisfying version should have been released (in the npm registry) before the application snapshot time. For example, an application can specify a versioning constraint (``P:$>$1.0.0'') at the snapshot May 2016. Hence, the actual installed version is the latest version that is greater than 1.0.0 and also has been released in the npm registry before May 2016.
This step allows us to find the installed version of the dependency at the analyzed snapshot time.
\\
%to resolve the dependency versioning constraint at the analysed snapshot time using
%The semver tool is the mechanism used by npm to resolve package dependencies.
%We find the actual installed version that satisfies the versioning constraint with an additional restriction, the satisfying version should have been released (in the npm registry) before the analysed snapshot time. 
%\emad{this step is very hard to follow. Just say what you do in a simple manner and then give an example maybe.}

\noindent
{\textbf{Step 2. Identify vulnerable dependency versions.}}
After determining the resolved (and presumably installed) version at the analyzed snapshot time, we check whether the resolved version is vulnerably or not. To do so, we check the advisories dataset for the versions that were available at that snapshot point.
If the resolved version is covered by the advisories dataset, we label it as a vulnerable dependency version. We skip the whole next step if the dependency version has not been mentioned in any advisory, i.e., the dependency version is not vulnerable.
\\

\noindent
{\textbf{Step 3. Identify threat levels of vulnerable versions.}}
Once we identify the vulnerable dependency versions at the analyzed snapshot time, we classify each vulnerable dependency version using one of the threat levels we defined earlier (in Section~\ref{sec:ex}), i.e., we find out the threat level of each vulnerable dependency version. To do so, for each vulnerable version, we compare its vulnerability \textit{discovery (report)} and \textit{publication} time to the analyzed snapshot time. As we stated previously (in Section~\ref{sec:ex}), if the vulnerability publication time of the vulnerable dependency version is before the application's snapshot time then we mark the vulnerability as high threat vulnerability. If the vulnerability of the dependency was not published but only discovered (reported) before the application's snapshot time, then we mark it as medium. And finally, if it was neither published nor discovered (reported) before the analyzed snapshot time (i.e., no one knows about it at that snapshot time), then we mark it as low. %\emad{this last bit is repetitive. if we need space, we can remove it.}


In cases where more than one vulnerability affects the vulnerable dependency version, we resort to a weakest link approach (i.e., we label the vulnerable dependency version with the highest threat level). For example, if we find that the vulnerable version of the dependency is affected by two vulnerabilities -one having low threat and another as high threat, we label the vulnerable dependency version as high at that snapshot time.

\subsection{Replication Package}
To facilitate verification and advancement of research in the field, a replication package comprising the data used in our study along with the analyses used in our study is publicly available\footnote{http://doi.org/10.5281/zenodo.3837397}.

==> npm Vulnerability Threats/discussion.tex <==
In this section, we first address the cost of migrating dependencies
for a safer version (Section~\ref{sec:cost}). Then, we discuss how our findings
of vulnerable dependencies may lead to implications to researchers
and practitioners (Section~\ref{sec:imp}).
\vspace{-0.05in}
\subsection{Security Migration Cost}
\label{sec:cost}
Developers of Node.js applications may use dynamic versioning
constraints if they want to install the latest version of a dependency,
allowing them to get the latest updates for security fixes of the package. In fact, npm adopts a semantic version scheme~\cite{semvernp91}, where
package maintainers are encouraged to specify the extent of their
updates in three different levels: 1) patch release, which indicates backward compatible bug fixes, 2) minor release, which indicates backwards
compatible new features and 3) major release, which informs developers of
backwards incompatible changes in the package release. While our
study (RQ$_3$) showed that 90.76\% of high-threat vulnerabilities have a safe
version available for application maintainers (at the snapshot 100\%),
we manually inspected the fixed versions and the applications version constraints and found that in 43.07\% of the cases, the fix is only
available in another major release. For instance, an application
depends on P:1.0.0, and the fix patch was only released for a major
version 2.0.0 and onwards. Hence, to benefit from a fix patch in such a case, developers are required to upgrade their dependencies at the risk of breaking their own code, since a new major release has breaking
changes compared to the version the application depends on. This
imposes significant migration costs, especially for large projects
that depend on dozens of packages. Furthermore, this shows that
using dynamic versioning at the level of patch and minor releases
(as recommended by npm) does not completely prevent high threat
level vulnerabilities for affecting Node.js applications.

\vspace{0.1in}
\subsection{Implications}
\label{sec:imp}
%Our study provides solid empirical evidence on the prevalence of vulnerable dependencies and their respective threats levels to Node.js applications. 
%Researchers can utilize the results of our study to provide real statistics on the prevalence of vulnerable dependencies in the affected applications that depend upon them and their threats.
\textbf{Implications to researchers.}
Several studies have addressed the problem of vulnerabilities in software libraries~\cite{decan2018impact,zapata2018towards}. 
Our study, however, complements previous studies by analyzing the risks of vulnerable dependencies in the Node.js applications, aggregating the vulnerability lifecycle through the threat level metric.

%focus on the threat of vulnerable dependencies at the application level, viewing the security problem in ecosystems from a different perspective. 
Researchers can use our empirical evidence to better understand the risks Node.js applications face due to their high reliance on dependencies. 
%A recent study by Decan et al.~\cite{decan2018impact} shows that vulnerabilities take a very long time to be disclosed and published. On the other hand, Zapata et al.~\cite{zapata2018towards} found that projects are mostly safe because they don't touch the vulnerable functionality of their dependencies. 
%However, in our study, we conduct our analyses at a higher abstraction than the API level, i.e., we focus on the threat of vulnerable dependencies in the dependent client applications; to better understand the degree to which Node.js applications rely on vulnerable dependencies and understand how threatening such vulnerable dependencies really are in through dependent applications lifetime in the context of npm ecosystem. 
%We define three threat levels for vulnerabilities based on their lifetime. 
Our results show that most vulnerable dependencies found in a application snapshot have a low risk of being exploited when considering the lifecycle of vulnerabilities and how applications update their dependencies. Our results also show that the time element is crucial to understanding the threat of vulnerable dependencies in applications. 
 
Hence, a major implication of our study for researchers is that not all vulnerabilities are equal, and should not be treated and analyzed as such. 
Research needs to account for more than the existence of  vulnerabilities to draw more meaningful analyses regarding software security, particularly for applications in software ecosystems where the level of dependency continues to increase. Research can use our threat-level approach to provide a more refined picture when reporting the impact of vulnerabilities. Researchers can also reuse our approach to help them identify and classify vulnerable dependencies in the applications (in Section~\ref{subsec:scanning}).
%, which be employed to obtain more refined picture of the danger of vulnerabilities in software dependencies.
%
%
%The code and dataset used in this analysis is available at \diego{link?.}

Furthermore, more studies across ecosystems are necessary to get a broader perspective on the threat level of vulnerability  dependencies.
npm is one of the largest ecosystems and since applications depend on an increasingly high number of packages~\cite{decan2018empirical}, Node.js applications may be subjected to higher risk of vulnerable dependencies.
Further investigation could unveil if this pattern holds in other ecosystems.
\\

%that application developers need to take updates pushed from their dependencies seriously, or at least actively track their dependencies, since those can lead to very serious effects. To help in doing so, our approach to identify and classify vulnerable dependencies in the applications (in Section~\ref{subsec:scanning}) can be employed to help developers and researchers monitor security status and vulnerabilities in the applications with a realistic criteria of safety (threat levels), for vulnerabilities, given the dependency constraints by modern package managers (i.e., versioning constraints).
%\mhmd{Example: no studies discuss how developers manage/prioritise their dependency vulnerabilities. Is it the popularity, usage, or frequently affected dependencies?
%warnings for vulnerability in dependencies are overblown and that a lot of these vulnerabilities cannot be threat the dependent applications, leading only to notification fatigue for developers who get bombarded with warnings that seem not very relevant to them. Hence, we need models for prioritizing}

%\implication for developers: developers should not assume that all npm dependencies packages are of  high threat since our findings show otherwise. npm packages are expect are grwoing rapidly, making the task of monitoring their vulnerabilities even harder. Hence, the issue of how to manage and help developers prioritize their dependency vulnerabilities needs to be addressed. To some extent, npm-audit has been   recently adopted by npm to specically scan all published depednency vulnerabilities. However such tool  provide an abstract status
\noindent
\textbf{Implications to practitioners.}
Our results revealed important takeaways for software practitioners.
First, vulnerable dependencies are common, 67.93\% of the studied Node.js applications had at least one vulnerable dependency at the last studied snapshot.
Practitioners need to be in constant alert to update their dependencies and tools that increase awareness of vulnerabilities, such as Dependabot~\cite{Dependab26:online} and \texttt{npm audit}~\cite{npmaudit59:online} are evermore crucial for the safety of software applications, especially because they warn developers as soon as the vulnerability becomes of a high threat level.

Second, practitioners also need to account for the threat level of a vulnerability to have a more correct understanding of software vulnerabilities in software ecosystems. Our method of analysis can also be used by developers to identify packages that more often raise the threat level in their applications.
Also, while vulnerabilities are widespread in open-source packages in the npm, in most cases package maintainers issue a fix patch for their vulnerability as soon as it becomes public, which is crucial to mitigate the chances of having a vulnerability exploited and cause potential harm to end-users and application maintainers.

Third, our study showed that developers are in need of more tools that go beyond simply warning them of a published vulnerability. For example, they need tools to help them understand: 
1) the costs of migrating to a safer version and whether it is possible to fix a vulnerability without breaking their code,
2) the frequency in which certain dependencies have become vulnerable in the past, in order to grab the threats of depending on such packages and better plan their project maintenance,
3) history of all vulnerable dependencies of their application in order to understand the frequency and the duration in which their application became at the risk of a high threat vulnerability in the past. 
Packages that do not update their code to address reported vulnerabilities incur in a high risk for applications that use them and should be avoided by critical applications.
%Moveover, vulnerable dependencies information may be regularly collected by such a tool to build history of the frequent vulnerable dependencies over the application lifetime and learn from it to mitigate their threat in the future.
%
%2) the threat of vulnerable dependencies at any historical point in time of the application, (using our defined classifications, for example), to build quite rich information about vulnerable dependencies in their applications.
%2) whether it was possible to fix a vulnerable dependency by just a simple patch update (e.g., measure the risk of incompatibility),
%
%
%
%\textbf{Tools for checking the health of npm dependencies in the history of dependent applications.}
%Existing tools (e.g., {\fontfamily{qcr}\selectfont \npm audit}) provide application developers with an abstract status of the npm vulnerable dependencies in the applications, meaning that such tool doesn't provide a history of the vulnerable dependencies in the dependent applications and how threatening they are at a specific point in time. 
%\textbf{Tool builders should consider supplying application developers with enhanced tools to help them understand:}
%(1) the threat of vulnerable dependencies at any historical point in time of the application, (using our defined classifications, for example), to build quite rich information about vulnerable dependencies in their applications.
%(2) whether it was possible to fix a vulnerable dependency by just a simple patch update (e.g., measure the risk of incompatibility),
%(3) whether certain vulnerable dependency occurred frequently in the past, 
%and (4) individual statistics (history) of vulnerable dependencies in order to determine whether some packages require special treatment or maintenance.
%Vulnerable dependencies information may be regularly collected by such a tool to build history of the frequent vulnerable dependencies over the application lifetime and learn from it to mitigate their threat in the future.

==> npm Vulnerability Threats/introduction.tex <==
%software vulnerabilities are bad. Ton of them around and exaborated in software ecosystems
The existence of a software vulnerability in a software system is a major concern for software projects. These vulnerabilities can cause unimaginable damage for an organization if exploited. In fact, there are many examples of such cases. 
One such example is the Equifax cybersecurity incident~\cite{EquifaxR95}, where a vulnerability in Apache Struts led to unauthorized access to consumers' personal information and credit card numbers.

To make matters even worse, the recent popularity of software ecosystems has only magnified the problem. Specifically, most software systems today have many direct and transitive dependencies, which increases the risk of a vulnerability in a software project. Contrast Security, a software security company, reported that 80\% of the code written in today's applications depend on external packages, and approximately one fourth of package downloads have known vulnerabilities~\cite{williams2012unfortunate}. Furthermore, a recent report by Snyk.io showed that 83\% of organizations use vulnerable packages and that 77\% of the 430,000 websites crawled by them, run at least one vulnerable JavaScript package~\cite{77of433093:online}.
%Zimmermann et al.~\cite{zimmermann2019small} studied security threats in the npm ecosystem by mainly analysing the maintainers role and their  responsibilities for vulnerable packages. They mainly observed that a very small number of maintainers' accounts (i.e., 20 accounts) could be used to  threaten large code bases by injecting malicious code into thousands of npm packages. 
These reported figures are worrisome given our everyday dependence on software systems.
 
%yet, software systems are everywhere and seem to be functioning OK for the most part. so we argue that although this doom and gloom of software vulnerabilities makes for good marketing, not all vulnerabilities are treated equally.
However, although these vulnerability reports are worrying, they impact a very tiny fraction of existing software systems~\cite{pashchenko2018vulnerable,zapata2018towards}.
%\diego{Since this is a bold claim, it would be great to have more references.}
For example, a recent study manually analysed 60 projects that depend on high severity vulnerabilities, and found that 73.3\% of them were actually safe because they didn't make use of the vulnerable functionality of their dependencies~\cite{zapata2018towards}.
%
%%However, 
%the reality we observe is very different. Although these reports are worrying, the reality is most software systems function just fine. 
%\diego{This is a bold statement. If we start with such statements we need to deliver a high-quality payoff, as we seem to be challenging some of the "beliefs" of the security community.}
%In the grand scheme of things, these vulnerabilities impact a very tiny fraction of existing software systems. A recent study \cite{zapata2018towards} has manually analysed 60 projects that depend on high severity vulnerabilities, and found that 73.3\% of them were actually safe because they didn't make use of the vulnerable functionality of their dependencies.

Hence, we argue that \emph{not all vulnerabilities are equal}. To get the real picture, one needs to take into consideration the \emph{potential threat} of a software vulnerability. Formally defined, the threat of a vulnerability is {the potential danger to exploit a vulnerability in order to breach security and cause possible harm}~\cite{shirey2000internet}.


%``possible danger that arises from the exploitation of a vulnerability to breach security and cause possible harm''~\cite{shirey2000internet}.




%OWASP, an organization focused on improving the security of software, defines several factors that estimate such threat~\cite{OWASP}. \textit{How well known is the vulnerability to a threat agent}), is one of these factors.%, where a vulnerability is assigned a \textit{low} threat level if it was hidden or still unknown at the time one checks for vulnerabilities (\textit{t}), \textit{medium} threat level if the vulnerability is reported but not yet published at \textit{t}, and \textit{high} if it is publicly announced at \textit{t}.

%define what we do, i.e., low, med, high
The main goal of our study is to examine the degree that applications rely on vulnerable dependencies and understand how threatening such vulnerable dependencies really are. To achieve our goal, we first provide a threat classification for the software vulnerabilities based on their lifecycle. Note that this is a post-mortem classification, using information only available after the fact, for the purpose of evaluating the threat of dependency vulnerabilities in the dependent applications. We classify software vulnerabilities into three main threat levels: \emph{low threat}, indicating that a vulnerability that affects a dependency was not discovered (reported) yet at a specific point in the application lifecycle; \emph{medium threat}, indicating that a vulnerability was discovered but not yet published (publicly announced); \emph{high threat}, indicating a vulnerability has been published. %and/or a proof-of-concept of how to exploit it is given.

%What we do and what we find
We use our classification and perform an empirical study involving 6,673 real-world, active, and mature open source Node.js applications, of which more than half have at least one vulnerable dependency. We use these classifications to examine {(RQ1) how threatening vulnerable dependencies in the dependent applications really are,} (RQ2) how the threat levels of vulnerable dependencies evolve through the applications development history, and (RQ3) why some applications end up depending on high threat vulnerabilities in order to better understand how we can mitigate such issues. %Hence, we formulate the following three research questions:
%\begin{itemize}
%	\item   \rqone
%		\item   \rqtwo
%			\item   \rqthree
%\end{itemize}

Our findings show that although 67.93\% of the examined applications have (in one of their recent versions) at least one vulnerable dependency, 94.91\% of the vulnerable dependencies in these applications are classified as having low threat (RQ1). Moreover, as applications evolve, they are more likely to depend on vulnerable dependencies, however, most of the vulnerabilities have a low threat level (RQ2). Lastly, we find that the vast majority (90.8\%) of the high threat dependency vulnerabilities were caused by the applications, i.e., vulnerable dependencies had an available vulnerability fix but the applications did not update to a newer (safer) version of the vulnerable dependency (RQ3).

%When considering the entire development history of the applications, i.e., other application versions than the recent studied version, we observed that the number of affected applications overall increased from 55.31\% at an earlier point of their lifetime up to 67.93\% for the applications' last studied version, actually showing an increasing in vulnerable dependencies across the applications' lifetime due to the increasing of overall number of dependencies in the applications. 

%Once again, we also observed that vulnerable dependencies still have low threat on the applications even when considering different points in the applications development history (RQ2).

%In other words, the vulnerability was not known at the time of adding the dependency of the vulnerable package version, and an exploit was not available for it. 

%90.8\% of the high threat dependency vulnerabilities were caused by the applications, i.e., vulnerable dependencies had an available vulnerability fix but the applications did not update to a newer (safer) version of the vulnerable dependency, and this observation still holds when considering different points in the applications development history (RQ3).

% the contributions later.
As a key contribution, we provide an empirically-sound evidence regarding the degree to which Node.js application projects rely on npm vulnerable dependencies and how such vulnerable dependencies are threatening through applications development history, while also discussing the implications of our findings to researchers and practitioners. Besides, we provide an approach to identify vulnerable dependencies in a Node.js application at a given point in time, taking into consideration our vulnerability threat classification. Other researchers analysing vulnerabilities in npm dependencies can reuse it. Finally, we provide a replication package comprising the techniques and dataset that we used in this study as a means to bootstrap other studies in the area.

The rest of the paper is organized as follows. Section~\ref{sec:background} introduces our vulnerability classification used in this study. Section~\ref{sec:dependency} describes how npm manages dependencies in Node.js applications. Section~\ref{sec:case_study_design} describes our case study design. Section~\ref{sec:results} presents our results. Section~\ref{sec:discussion} discusses how our results lead to direct implications to researchers and practitioners. Section~\ref{sec:related_work} discusses the related work. Section~\ref{sec:threats} presents the threats to validity. Section~\ref{sec:conclusion} concludes our paper.

% npm fig
%\begin{figure}[!h]
%  \centering
%  \includegraphics[width=1\linewidth]{images/npm}
%  \caption[]{Growth in ecosystems.\footnote{http://www.modulecounts.com/}}
%  \footnotetext[4]{http://www.modulecounts.com}
%  \label{npm}
%\end{figure}

==> npm Vulnerability Threats/related_work.tex <==
The work most related to our study falls into two main categories - studies on software ecosystems and studies on security vulnerabilities in packages. In the following, we discuss the related work and reflect on how the work compares with ours.

\subsection{Software Ecosystems}
%%Intro
A plethora of recent work focused on software ecosystems. Several works compare different ecosystems. For example, Decan et al.~\cite {decan2018empirical} empirically compared the evolution of 7 popular package ecosystem using different aspects, e.g., growth, changeability, resuability, and fragility. They observed that the number of packages in those ecosystems is growing over time, showing their increasing importance. 
%Also, they concluded that considering different ecosystems in the analysis may reveal different findings depending on the characteristics of ecosystems.

%%\bram{interesting aspect, could this be related to your evolution results?}
Other work focused specifically on npm~\cite{fard2017javascript,kula2017impact, wittern2016look}. For example, Fard et al.~\cite{fard2017javascript} examined the evolution of dependencies within an npm project, and showed that there is a heavily interdependence, with the average number of dependencies being 6 and growing over time. Wittern et al.~\cite{wittern2016look} investigated the evolution of npm using metrics such as dependencies between packages, download count, and usage count in JavaScript applications. They found that packages in the npm ecosystem are steadily growing. Such amounts of packages make the spread and discovery of vulnerabilities much worse, given the heavy dependence on such packages and the potential security problems in those packages.
%

Other studies pointed out the fragility of software ecosystems and provided insights on the challenges application developers face. For example, Bogart et al.~\cite{bogart2015breaks,bogart2016break} examined the Eclipse, CRAN, and npm ecosystems, focusing on what practices cause API breakages. They found that a main reason for breaking changes are the updates of a dependency. This finding may explain why application developers are hesitant to update and explain why we see high threat vulnerabilities impacting applications that do not update in time. 
%
%\mhmd{rephrase:Begin}
%Additional studies have focused specifically on how developers manage dependencies and versions within environment configuration. Xavier et al.~\cite{xavier2017we} note that developers deliberately make breaking changes to APIs for several reasons related to code maintenance. Further, Dietrich et al.~\cite{dietrich2019dependency} found that developers struggle with different options for specifying dependency versions that are supported by many package management systems.\mhmd{rephrase:End}
%
%

Our study differs from the prior work since we focus on the threat level of dependency vulnerabilities in Node.js applications. Moreover, we examine how this threat level changes as applications evolve and examine the reason that high threat dependency vulnerabilities exist. That said, much of the aforementioned work motivated us to study npm and focus on examining vulnerabilities in application dependencies.
\vspace{-0.05in}
\subsection{Security Vulnerabilities in Dependencies/Packages}
%

% vulnerabilities in dependencies generally
Several works in the literature studied vulnerabilities that come from dependencies~\cite{di2009life,pham2010detection,cox2015measuring,massacci2011after,derr2017keep}. For example, Di Penta et al.~\cite{di2009life} and Pham et al.~\cite{pham2010detection} conducted empirical studies to analyze the evolution of vulnerabilities in source code, and found that most vulnerabilities are recurring due to software code reuse or libraries (i.e., dependencies). Cox et al.~\cite{cox2015measuring} evaluated ``dependency freshness'' to understand the relationship between outdated dependencies and vulnerabilities using industry benchmarks, and found that vulnerabilities were four times as much likely to have existed in outdated systems than in updated systems. Relative studies by Massacci et al.~\cite{massacci2011after} and Derr et al.~\cite{derr2017keep} are in line with~\cite{cox2015measuring}. In general, they both reported that vulnerabilities appeared commonly in non-maintained code and old versions, and this could be fixed by just an update to a newer version. Our study complements these studies by examining the threat of these vulnerabilities in the dependent applications.

 
%studies on vuln ecosystems with special on npm
More specifically, vulnerabilities that affect packages in ecosystems have been studied broadly~\cite{kula2018developers,pashchenko2018vulnerable}. For example, Kula et al.~\cite{kula2018developers} analyzed the Maven ecosystem on more than 4,000 GitHub projects that correspond to 850,000 library migrations, and found that projects were heavily dependent on these libraries, and most projects (i.e. 81.5\%) had outdated libraries. The study also mentioned (based on interviews conducted with developers) that developers do not update dependencies, and 69\% of the interviewed developers tend to be not aware of their vulnerable dependencies. Pashchenko et al.~\cite{pashchenko2018vulnerable} studied the vulnerability impact of 200 open-source Java libraries commonly used in SAP~\cite{SAPSoftw78} organisation, and found that 20\% of the vulnerable dependencies are not deployed, and hence, they are not exploitable in practice. Moreover, they found that the majority of the vulnerable dependencies (81\%) can be fixed by a simple upgrade to a newer safe version, suggesting that software development companies have to  allocate their audit tools correctly.

Other recent work focused on analyzing vulnerabilities in the npm ecosystem. For example, Hejderup’s~\cite{hejderup2015dependencies}
analysed only 19 vulnerable packages
and found that the number of vulnerabilities in them is growing over time. Similarly, Decan et al.~\cite{decan2018impact} analyzed the vulnerabilities in the npm ecosystem and found that the number of vulnerabilities is growing over time. Also, they reported that it takes a long time to discover vulnerabilities that affect npm packages. Our study complements this study by analyzing the risks of vulnerable dependencies in the Node.js applications (not addressed by the study~\cite{decan2018impact}), aggregating the vulnerability lifecycle through the threat level metric. 
A recent study by Zapata et al.~\cite{zapata2018towards} assessed the danger of having vulnerabilities in dependent libraries by analyzing function calls of the vulnerable functions.
They manually analyzed 60 projects that depend on vulnerabilities, and found that 73.3\% of them were actually safe because they did not make use of the vulnerable functionality of their dependencies, showing that there is a considerable overestimation on previous reports. Our study identifies yet another source of overestimation by including a time-based analysis into a large and comprehensive set of \textit{applications} (i.e., 6,673 Node.js applications).
Zimmermann et al.~\cite{zimmermann2019small} studied the security threat of the npm ecosystem dependencies by mainly analysing the maintainers role and responsibilities for vulnerable packages. They mainly observed that a very small number of maintainers' accounts (i.e., 20 accounts) could be used to inject malicious code into thousands of npm packages, a problem that has been increasing over time. Zerouali et al.~\cite{zerouali2019impact} studied npm vulnerable packages in Docker containers, and found that they are common in the containers, suggesting that Docker containers should keep their npm dependencies updated.
%

To assess the impact of vulnerable dependencies in the dependent Java applications, Plate et al.~\cite{plate2015impact} proposed an approach that provides a fine-grained assessment of the vulnerabilities that affect dependencies in dependent Java applications. In particular, the approach first determines whether or not the application makes use of the library that is known to be vulnerable. Then, the approach tries to determine whether or not the application executes the fragment of the dependency where the vulnerable code is located. Furthermore, Ponta et al.~\cite{ponta2018beyond} built upon their previous approach in~\cite{plate2015impact} to generalize their vulnerability detection approach by using static and dynamic analysis to determine whether the vulnerable code in the library is reachable through the application call paths. Their proposed approach is implemented in a tool called, Vulas, which is an official software used by SAP to scan its Java code.

% how our study is different from the literature
Our study focuses on analyzing the threat of npm vulnerabilities in dependencies, which affected applications that rely on them. In many ways, our study complements the related work since, (1) instead of studying security vulnerabilities that exist in packages, we particularly focus on the threat of such vulnerable packages by real-world open source applications; (2) we provide a threat classification for software vulnerabilities based on their lifetime, and we use our classification and perform an empirical study on Node.js applications.


==> npm Vulnerability Threats/results.tex <==
In this section, we present our case study results that answer our 3 research questions (RQ). For each RQ, we motivate the question, detail the approach used and present the results.

%The goal of this study is to understand the threat level of vulnerable npm dependencies. We examine the Node.js applications in our dataset to quantify how threatening vulnerable dependencies in the examined applications really are (RQ1), how such vulnerable dependencies are classified across the threat levels through applications development history (RQ2), and to understand who is responsible for the dependence upon high threat vulnerable dependencies (RQ3).

%Note that both research questions are evaluated on the latest snapshot of the analyzed applications. The discussion section revisits this decision. %\bram{the questions should at least be listed in the case study setup, otherwise not clear what the aim of the setup is}

\subsection*{\rqone}
\label{sec:RQ1}
{\textbf{Motivation}}:
Prior work showed that a significant amount of application code comes from third party packages, and a non-negligible amount of these packages are affected by known security vulnerabilities~\cite{williams2012unfortunate}. However, we argue that not all vulnerabilities should be treated equally. Hence, in this RQ we would like to quantify how many of our studied applications have at least one vulnerable dependency and what the threat level of these vulnerable dependencies is. Answering this question will help us understand the real risk/threat of vulnerable packages on the software applications.

%
%if these vulnerable packages are used in the applications before their vulnerability reports get announced publicly then their impact on the application can be neglected, i.e., the chance of the application being exploitable is actually low.
%In addition, if the applications use the fixed patch version of the vulnerable package once it is available, we shouldn't
%worry much about the impact of the vulnerable packages in the applications that use them. 
%In this RQ, we want to understand whether
%the exploitability of vulnerable packages used in the applications in our dataset is really high. We focus on the latest snapshot of the applications.
%Answering this question will help us understand the real risk of
%vulnerable packages on the software applications that make use of them.
%
%\begin{figure}[tb!]
%	\centering
%	\includegraphics[width=1\linewidth]{images/vulnDelta}
%	\caption[]{Two possible scenarios of applications lifespan.}
%	\label{vulnDelta}
%\end{figure}
%
\noindent
{\textbf{Approach}}: 
In order to perform an unbiased analysis, we need to account for vulnerability discovery time. Prior work showed that vulnerabilities in npm take on median 3 years to be discovered and publicly announced~\cite{decan2018impact}. As a consequence, selecting snapshots of our applications in 2019 will paint an incomplete picture, as most vulnerabilities recently introduced in the package's code would remain hidden for a median of 3 years. 

Since we collected the advisories dataset in May/June 2019, we chose to evaluate our applications as of May 2016 (3 years prior), which ensures that at least half the dependency vulnerabilities introduced in the code are reported in the current advisories dataset. %Note that all applications in our dataset have an activity before this date (i.e., May 2016).

%This RQ is evaluated on one snapshot of the analysed applications.  It is crucial we account for the vulnerability life-cycle and the time needed to discover and publish a vulnerability in the advisories to select an appropriate application snapshot. As shown in a previous study~\cite{decan2018impact}, vulnerabilities in npm take in median 3 years to be discovered and publicly announced. As a consequence, selecting snapshots of our applications in 2019 will paint an incomplete picture, as most vulnerabilities recently introduced in the package's code would remain hidden for a median of 3 years. 
%%We need to choose a snapshot of an application in a point-in-time where the vulnerable dependencies have had enough time to be discovered and published in the advisories dataset. 
%Therefore, as our advisories dataset collection took place during May 2019, we chose to evaluate our applications at \textit{May 2016} (3 years prior), which ensures that at least half the vulnerabilities introduced in the code are reported in current advisories dataset.


%In fact, the selection of the snapshot is of a special importance due to the vulnerability lifecycle and the amount of time needed to discover and publish a vulnerability in a package. For example, if we select the \textit{latest snapshot} of each application as our studied snapshot, the results might be biased since our Node.js applications have different lifetime, e.g., some applications have the latest snapshot as of 2019, others have their latest snapshot as of 2018, and so on. Given that npm vulnerabilities take, on median, 3 years to be discovered and publicly announced~\cite{decan2018impact}, 
%%applications that have their latest snapshot as of 2019 haven not had enough time for their vulnerable dependencies at that snapshot to be discovered and published, and hence, evaluating the applications at their latest snapshot is not the most correct way for our analysis.
%%Therefore, 
%we need to choose the snapshot point in time at which the vulnerable dependencies in the applications have had enough time to be discovered and published {in the advisories dataset.} Our advisories dataset collection took place during May 2019. Hence, we chose to evaluate our applications at \textit{2016 May}, which can ensure the vulnerability discovery and publication (i.e., least 3 years).

%\mhmd{@Diego: can you please check the text here? If you remember, this is the vulnerability delta we considered to remove the flaw in our old methodology. We need to assume that reviewers most likely never read about this before :(}
%In fact, analysing the applications at the selected snapshot (i.e., 2016 May) requires the application to be active around the period of 2016 May).
%%Our applications had at least a recent commit between January 2017 and December 2017, and 
%Hence, we exclude applications that have their creation dates after 2016 May.
%Figure~\ref{vulnDelta} shows two possible scenarios of applications' lifetime and whether each scenario is included in our evaluation. The first scenario (top figure) is an application that has a lifetime that includes our selected snapshot, and hence, it is included in our evaluation. The second scenario is excluded from our applications dataset since  the application creation date is 2018 January.
%After this step of filtration, we end up with 6,673 applications included in our evaluation.
%The 6,673 applications are still of quality, having 213 commits,
%11 dependencies, and 1,657 days of development lifespan, on median.

Then, we answer our RQ in two steps. First, we examine if the \textit{selected snapshot} of the application had at least one dependency that contains a vulnerability (irrespective of its threat level). 
Then, to determine the threat level of the vulnerable dependencies in the examined applications, we focus only on the set of applications that have at least one vulnerable dependency using the methodology described in Section~\ref{subsec:scanning}. 
In the second step, we quantify the number of vulnerable dependencies in the applications under each threat level. 
We first check the percentage of overall vulnerable dependencies in each application and illustrate their distribution using a Boxplot. We further analyze the distribution of these vulnerable dependencies across the threat levels and plot it using three Boxplots, one for each threat level. For example, an application could have 10\% of its dependencies as vulnerable at the analysed snapshot, and such percentage (i.e., 10\%) could be distributed across the threat levels as follows: 25\% of the vulnerable dependencies are classified as low threat, 60\% of them are classified as medium, and 15\% as high.

\begin{figure}[tb!]
	\centering
	%\setlength{\abovecaptionskip}{10pt}
	\includegraphics[width=1\linewidth,height=.85\linewidth]
	{images/RQ1_new.pdf}
	\caption{Boxplots showing the distributions of the percentage of overall vulnerable dependencies in the applications (left boxplot), and how these percentages are distributed across threat levels (right boxplot). N and M are the total number of dependencies and the total number of vulnerable dependencies, respectively.
	%\diego{Fix the labels}
	}
	\label{RQ1Perc}
	
\end{figure}
%
\noindent \textbf{Results}: 
Of the 6,673 studied applications \textbf{67.93\% (4533 applications) depend on at least one vulnerable dependency}. The affected applications contains a total of 10,154 vulnerable dependencies from 149 distinct vulnerable packages. The 149 packages comprises 23.21\% of the overall vulnerable packages in the npm advisories dataset.

Figure~\ref{RQ1Perc} shows the percentage of vulnerable dependencies per application (left boxplot), and the distribution of vulnerable dependencies at different threat levels (right boxplot). It shows that, on median, 14.29\% of the dependencies in the affected application (i.e., applications with at least 1 vulnerable dependency) are vulnerable. Also, Figure~\ref{RQ1Perc} shows that such percentage of vulnerable dependencies (i.e., 14.29\%) is distributed as follows: \textbf{94.91\% of the vulnerable dependencies are classified as low threat vulnerabilities}, 2.06\% of them are classified as medium, and 3.03\% are classified as high.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\vspace{0.08in}
\begin{table}[h!]
	\centering
	\caption{Mann-Whitney Test (p-value) and Cliff's Delta (d) for the different threat levels.}
	\label{stattest}
	\begin{tabular}{l|r|r}
		\toprule
		\textbf{Threat Levels} & \textbf{\textit{p}-value} &\textbf{ Cliff's Delta \textit{{(d)}}} \\ \midrule
		%\textbf{Threat Levels} & \textit{p}\textbf{-value} & \textit{{d}} \\ \midrule
		Low vs. Medium & 2.2e-16 & 0.984 (large) \\
		Low vs. High & 2.2e-16 & 0.970 (large) \\
		Medium vs. High & 2.2e-16 & 0.335 (medium) \\ \bottomrule
	\end{tabular}%
\end{table}
\vspace{0.08in}
%Based on the previous observations, vulnerable dependencies of low threat are observed the most often, followed by the high and medium threat levels.
To statistically verify our observation, we perform a one-sided non-parametric Mann-Whitney U test~\cite{mcknight2010mann} by comparing the distributions between the different threat levels. 
Table~\ref{stattest} shows the p-values and effect size values. We observe a statistically significant differences between (low and medium), (low and high), (medium and high), at p-value $<$ 0.05 for all comparisons. Furthermore, we observe, using Cliff's delta~\cite{cliff1993dominance}, a large effect size for the differences between low and medium, low and high. Also, we found a medium effect size for the difference between medium and high. This indicates that the differences between the different threat levels are statistically significant.\\
%\vspace{-0.2in}

\begin{mdframed}[roundcorner=5pt,linewidth=0.5mm,
	linecolor=black]
	\lipsum[0]
	\textbf{\textit{Our findings show that 67.93\% of the examined applications depend on at least one vulnerable package. However, the vast majority (94.91\%) of these dependencies have low threat.}
}
\end{mdframed}

\vspace{0.2in}
\subsection*{\rqtwo}
{\textbf{\\Motivation}}: Thus far, we have analyzed the vulnerability threats of a single snapshot of each application in our dataset. However, our findings may differ as the applications evolve. For example, a vulnerability with high threat on a given day could have had low threat the week before.

%Hence, this RQ we re-examine the threat of vulnerabilities in two ways: 
%(1) we examine the threat levels of vulnerabilities that affect dependencies at different stages of the application's development history; (2) we divide the applications based on their age and examine the threat levels of their dependencies.

\begin{figure*}[tb!]
	\centering
		\setlength{\abovecaptionskip}{10pt}
	\includegraphics[width=1\linewidth]
	{images/RQ2Evol3_new.pdf}
	\caption{Boxplots showing the percentage of overall vulnerable dependencies and their distribution in each threat level over the studied snapshots. N and M are the total number of dependencies and the total number of vulnerable dependencies, respectively.}
	\label{RQ2Evol}
\end{figure*}


%\noindent\uline{Application Evolution vs. Threat Levels}

Hence, in this RQ we would like to determine whether our results generalize to different historical snapshots in the application's development lifetime. Such an evolutionary examination allows us to discover whether the trend of the threat levels changes across different stages of an application's lifetime.
\\
\noindent
{\textbf{Approach}}:
Since the different applications are of different lifespans, we want to find a measure that makes comparing them feasible. To do so, we use the number of commits as a way to divide the applications into different intervals. Since commit frequency and time between commits vary from one application to another, we normalize the applications by segmenting the lifetimes of each application into five equal intervals (each containing 20\% of an application's lifetime by {time in days}),
%~\diego{each containing 20\% of the commits?}, 
%\mhmd{No, we take first and last commit date, then find the duration in between, divide this duration into 5 time ranges and find the latest commit in each time range, and consider it a snapshot. Hence, it is 20\% from the application lifetime }
%\mhmd{I think we should explain the approach in detail}
take one snapshot at each interval, then analyze it. Although this might seem like a straightforward task, it poses some challenges, since we have a large applications dataset and the package.json file in them is updated significantly over the application's lifetime.
%, stressing on the amount of processing time it took for this analysis.
For this analysis, we only consider the affected applications identified in RQ$_1$.
%The analysed applications in this RQ are the affected applications that are identified in RQ$_1$.
The last snapshot (at 100\%) is the same snapshot that we analyzed in RQ$_1$ (i.e.,  May 2016).
%
%\begin{table}[tb!]
%	\centering
%	\caption{The percentage of vulnerable and non vulnerable applications at different historical snapshots. \emad{Please remove the non-vuln...obviously it is 100-vuln}}
%	\label{DisT1}
%	%\resizebox{\linewidth}{!}{%
%	%\small
%	\begin{tabular}{l|r|r}
%		\toprule
%		\multirow{2}{*}{\textbf{Snapshot}} & \textbf{Vulnerable} & \textbf{Non Vulnerable} \\ 
%		&	\textbf{Applications} &	\textbf{Applications}\\
%		\midrule
%		\textbf{20\%} &{ 55.31\%} & {44.69\%} \\
%		\textbf{40\%} & 58.17\% & 41.83\% \\
%		\textbf{60\%} &  60.87\% & 39.13\% \\
%		\textbf{80\%} &  63.03\% & 36.97\% \\
%		\textbf{100\%} & {67.93\%} & {32.07\%} \\ \bottomrule
%	\end{tabular}%\hlc[lightgray]
%	%}
%\end{table}

\begin{table}[tbh]
	\centering
	\caption{The percentage of vulnerable applications at different historical snapshots.}
	\label{DisT1}
	%\resizebox{\linewidth}{!}{%
		%\small
		\begin{tabular}{l|r}
			\toprule
		\multirow{2}{*}{\textbf{Snapshot}} & \textbf{Vulnerable}  \\ 
										&	\textbf{Applications} \\
			\midrule
			\textbf{20\%} &{ 55.31\%}  \\
			\textbf{40\%} & 58.17\%  \\
			\textbf{60\%} &  60.87\%  \\
			\textbf{80\%} &  63.03\%  \\
			\textbf{100\%} & {67.93\%} \\ \bottomrule
		\end{tabular}%\hlc[lightgray]
	%}
\end{table}
\noindent
{\textbf{Results}}:
Table~\ref{DisT1} shows the percentage of applications that have at least one vulnerable dependency for the 5 analyzed snapshots across their lifetime. We observe that \textbf{the percentage of vulnerable applications steadily increases each snapshot} and varies between 55.31 - 67.93\% in the studied applications.

Figure~\ref{RQ2Evol} illustrates the distributions of the percentage of vulnerable dependencies at each threat level over the studied snapshots. The total number of dependencies (N) and the total number of vulnerable dependencies (M) in the studied applications are shown at the bottom of Figure~\ref{RQ2Evol}. The raw numbers of the dependencies show that the total number of dependencies increases over time, and so does the raw number of vulnerable dependencies.

From Figure~\ref{RQ2Evol}, we observe that the affected applications depend on vulnerable dependencies at an earlier stage (i.e., at 20\%) of their lifetime. However, we also observe that the trend observed in RQ1 remains the same, i.e., the overall percentage of vulnerable dependencies ranges between 14.29\% - 14.68\%. Also, the majority of the vulnerabilities have a low threat level, followed by high and medium threat. To sum up, our analysis shows that all trends observed in RQ$_1$ %Section~\ref{sec:RQ1} 
also hold at different stages of the applications, albeit the raw number of dependencies does increase.\\
%To statistically verify our previous observations over the studied snapshots, we perform one-way ANOVA~\cite{kruskal1952use} (a.k.a Kruskal–Wallis), a non-parametric method for comparing two or more distributions of equal or different sizes. We found that no significant difference among severity levels. P-value of Kruskal test is \mhmd{WIP} at 95\% confidence level

%\noindent\uline{Application Lifespan vs Threat Levels}
%{\textbf{\\Motivation}}:
%Although our earlier analysis showed that the threat trends hold at the different stages of an application, it still remains unanswered whether the age of the applications impacts our findings. For example, do older applications tend to have more medium and high threat vulnerabilities than younger applications, and vice versa? 
%This examination also allows us to better understand the phenomena of application maturity vs. threat of vulnerable dependencies.
%%This question is important to investigate, especially given our findings in RQ2, which showed that when it comes to high exploitability vulnerabilities, the applications depending on older versions seem to be the main cause.
%
%\noindent
%{\textbf{Approach}}:
%To understand whether the age of the applications impacts our findings, we split the studied applications into two groups - older and younger applications. To make this divide, we measured the median age of the studied applications, which we determined to be 1,657 days, and used that as a divider for the studied projects. 
%%using the median age of 1,657 days found in Section~\ref{subsec:data}. 
%%\diego{Where was this discussed?}
%The first group, which we call the young applications, are applications that are less than or equal to 1,657 days and the older applications are the ones older than 1,657 days. Of the 4,533 affected applications, 46.23\% are considered to be young applications and 53.77\% are old applications. 
%
%When examining the differences between the two sets of applications, we use the Mann-Whitney U test~\cite{mcknight2010mann} to ensure that the differences we observe are statistically significant. %comparing the distributions between old and young applications in each threat level across the different snapshots (pair-wise).
%
%%young
%%\begin{figure*}[tb!]
%%	\centering
%%	\includegraphics[width=1\linewidth]
%%	{images/RQ2EvolYoung.pdf}
%%	\caption{Boxplots showing the percentage of overall vulnerable dependencies and their distribution in each exploitability level over the studied snapshots for \textit{\textbf{young}} applications.}
%%	\label{RQ2EvolYoung}
%%\end{figure*}
%%%Old
%%\begin{figure*}[tb!]
%%	\centering
%%	\includegraphics[width=1\linewidth]
%%	{images/RQ2EvolOld.pdf}
%%	\caption{Boxplots showing the percentage of overall vulnerable dependencies and their distribution in each exploitability level over the studied snapshots for \textit{\textbf{old}} applications.}
%%	\label{RQ2EvolOld}
%%\end{figure*}
%\noindent
%{\textbf{Results}}:
%Our results show no statistically significant difference (p-value > 0.05) between old and young applications, confirming the observed trends in RQ$_1$ (in Section~\ref{sec:RQ1}), for applications of different ages. We present the respective distribution of threat levels for young and old applications in Appendix. \emad{NO, we need to add the results here. This is not goning to fly...}
%\\
%showing that  \textbf{as the applications evolve, the majority of vulnerabilities that affect the dependencies are of low threat}, confirming the observed trends in RQ$_1$ (in Section~\ref{sec:RQ1}) for applications of different lifespans. Also, the statistical analysis test we perform shows no significant difference. We present the respective Figures that present our results (in Appendix)
%Figures~\ref{RQ2EvolYoung} and ~\ref{RQ2EvolOld}  shows the distribution of threat levels for young and old applications, respectively.

%We observe, that \textbf{for both young and old applications the low threat vulnerabilities are the majority followed by high and medium exploitability, respectively}. That said, we again see that \textbf{as the applications evolve, the majority of vulnerabilities that affect the dependencies are of low threat}, confirming the observed trends in RQ$_1$ (in Section~\ref{sec:RQ1}) for applications of different lifespans.\\

\begin{mdframed}[roundcorner=5pt,linewidth=0.5mm,
	linecolor=black]
	\lipsum[0]
	\textbf{\textit{As applications evolve, the overall number of vulnerable dependencies is increasing, however, the median percentage of vulnerable dependencies remains mostly constant. Moreover, the majority of vulnerabilities they face remain as low threat vulnerabilities, as these applications evolve.}}
\end{mdframed}

\vspace{-0.2in}
\subsection*{\rqthree}
\textbf{Motivation}:
In the previous research questions, we found that the majority of affected dependencies are impacted by low threat vulnerabilities, throughout applications development history.
%\diego{We need to decide to go as simply low threat or low threat impact.}
However, a sizeable number of projects depend on  %medium and 
high threat dependencies, which are the most important. This means that those applications depend on vulnerable versions of dependencies even after the vulnerability reports have been discovered (reported)-and-published.
In such cases, the \emph{developers of the applications could know} about the presence of the vulnerability in the dependency, and hence, {should} avoid using that vulnerable version, if a fix is available.
%\diego{How would developers know in the case of medium threat? Aren't these cases only evident to the package developers and npm advisories?}
Specifically, we want to know who is to blame - the package maintainers for not providing a version that fixes a known vulnerability - or the application maintainers for not keeping their applications up-to-date. 
Answering this will help us pinpoint the causes for high threat vulnerabilities in npm applications and develop further strategies to solve this problem. 

%improve our understanding, so that such cases can be minimized in the future.

\noindent
\textbf{Approach}:
%Note that this RQ is most justified to be analyzed only for the high threat vulnerable dependencies (also for medium, but the medium category is already too low in number that any further analysis on them doesn't make much sense). 
%\diego{I am a bit confused. Is this last setence supposed to be a comment? :)}
%Therefore, we conduct our analysis only for high threat vulnerable dependencies. Furthermore, for consistency, we consider the analysis over the same five snapshots studied in RQ2.
%
To perform our investigation and answer who is responsible for the high threat vulnerabilities in applications, we use the same method to determine high threat vulnerabilities as presented in the first two RQs.
%To perform our investigation and answer who causes high threat of vulnerabilities (i.e., whether the vulnerable dependencies had an available fix at the studied snapshot time but not patched in the application),%why an application depends on a vulnerable version of the package, 
%we determine all versions/times where a package was vulnerable and not vulnerable. To do so, we utilize our collected advisories dataset (in Section~\ref{subsec:data}), which specifies all the safe versions of a vulnerable package, which we associate with the release time of each safe version from the npm registry. 

%. For each vulnerability, we identify the list of all safe versions of that vulnerability in the vulnerable package along with the version's release time.
%
%\textit{patches range} information available from the npm advisories dataset (described in Section~\ref{sec:case_study_design}). The \textit{patches range} 
%\diego{Revisit this paragraph. Patches range seems like a bad term and we have removed this term in the methodology section.}

%Then, we perform the analysis on the high threat vulnerable dependencies in each application. 
For each high threat vulnerable dependency, we check the availability of a safe version of the package for the vulnerability at the analyzed snapshot time. Depending on such availability our analysis has one of two outcomes:
\begin{itemize}
	
	\item \textbf{Package-to-blame:} if at the analyzed snapshot, no safe version has been provided by the package maintainers for a publicly known vulnerability. As the publication of a vulnerability comes after a period of 45 days, we consider the package maintainers the responsible for the high threat vulnerability in applications.
	
	\item \textbf{Application-to-blame:} if there is already a released safe version of the vulnerable package but the application continues to rely on an (old) version with a publicly known vulnerability.
	Application developers should monitor their dependencies and update to releases without known vulnerabilities, hence, we consider the application maintainers as responsible for the high threat vulnerability. 
	

\end{itemize}

% which would indicate the \textbf{package} is to blame. % if such a safe version does not exist at the snapshot time a dependency was used in the application. 
%Specifically, using the safe versions, we check whether the safe version's release time comes before the analysed snapshot time. Otherwise, i.e., a fix version is available but not patched by the application, it is possibly indicating that the \textbf{application} is to blame when such a safe version can be found.

%Second, when a safe version is available, we check whether the safe version would satisfy the dependency semantic versioning constraint defined by the application, possibly indicating that the \textbf{application} is to blame when such a safe version can be found.


\begin{table}[tb!]
	\centering
	\caption{The percentage of vulnerabilities caused by the lack of available fix patch (Package-to-blame) vs caused by the lack of dependencies update (Application-to-blame), over the applications snapshot.}
	\label{RQ2T1}
	%\resizebox{\linewidth}{!}{%
		\begin{tabular}{l|r|r}
			\toprule
			\textbf{Snapshot} &
			\textbf{Package-to-blame} &  \textbf{Application-to-blame} \\
			\midrule
			\textbf{20\%} & {12.06\%} & {87.94\%}  
			\\
			\textbf{40\%}  &  {9.52\%} & {90.48\%} \\
			\textbf{60\%}  & 11.91\% & {88.09\%} \\
			\textbf{80\%}  &  {12.43\%} &{87.57\%} \\
			\textbf{100\%}  & \textbf{9.24\%} & \textbf{90.76\%} \\
			\bottomrule			
		\end{tabular}%
%	}
\end{table}

\noindent
\textbf{Results}:
Table~\ref{RQ2T1} shows the percentage of high threat vulnerabilities based on our responsibility analysis. From Table~\ref{RQ2T1}, we observe that \textbf{for high threat vulnerabilities, the application is to blame in 90.76\% of the cases} at the last snapshot (i.e., 100\%).
That means that in 9 out of 10 cases the high threat vulnerability had an available fix, but the applications did not update their dependencies to receive the last fix patch.
%i.e., such percentage of  high threat vulnerabilities had an available fix at the snapshot time but not patched by the application}.
Note that this observation holds over all snapshots, with percentages of application-to-blame cases varying from 87.94\% to 90.76\%.
%\diego{I think we need to use a better term than ``reason". A package represents a high threat because it is vulnerable and people know about it (this is the reason). Now, the responsible for the high threat in the application can be either the package or the application. We need to update RQ3. }

Therefore, and perhaps counter-intuitively, high threat vulnerabilities do not exist because packages have unfixed vulnerabilities, rather the real cause is the fact that these applications fail to keep up or at least to inform themselves well enough about a given dependency version. Hence, a major implication of our study is that application developers need to take updates pushed from their dependencies seriously, or at least actively track their dependencies, since those can lead to very serious effects.

%At the same time, we do see that for medium exploitability vulnerabilities, the majority are due to the lack of packages being fixed and released in time, hence package maintainers need to make sure that they provide fixes in time for vulnerabilities before they are published and a proof-of-concept of the vulnerability is widely known.

It is important to note that we do not argue about the severity of the vulnerabilities, but rather their likelihood threat of being exploited. Hence, a low severity vulnerability can be very dangerous if everyone knows how to exploit it (high threat level according to our classification). The inverse is also true in that a high severity vulnerability can have a very low chance of being exploited if no one knows about its existence (low threat level).\\
\begin{mdframed}[roundcorner=5pt,linewidth=0.5mm,
	linecolor=black]
	\sloppy
	\lipsum[0]
		\textbf{\textit{{Our findings show that applications not updating their dependencies, are the main cause of high threat (more than 87\%) vulnerabilities.}}
	}
\end{mdframed}

==> npm Vulnerability Threats/threats.tex <==
%We now discuss the threats to the validity of our study. Our study, as all empirical studies, is subject to some threats to validity.
\textbf{Construct Validity} considers the relationship between theory and observation, in case the
measured variables do not measure the actual factors. Our dataset contains 654
vulnerabilities available in the npm advisories dataset. There might be other vulnerable packages that have been discovered but not yet reported. However, we leveraged up-to-date dataset from npm advisories, which we believe contains complete information about the vulnerable packages reported to them.

With respect to the affected dependencies, we only take into consideration production dependencies (i.e., dependencies that are required to install and run the application). We ignore other types (e.g., development dependencies), because they have no direct impact on the production environment.

This paper only considered direct dependencies. Our results may vary if indirect dependencies are considered, however, due to computation requirements, we focused on the direct dependencies of applications. In the future, we plan to expand our technique to consider indirect dependencies when considering the threat of vulnerabilities.

We did not consider whether the vulnerable functionality in the package actually affects the application, i.e., whether the applications uses the vulnerable code of the package. Considering this would be challenging, since our dataset is composed of thousands of applications. That said, our analysis is in line with prior work in the area of software ecosystems, which also examine dependencies in the package.json file to associate packages to applications.
\\

\noindent \textbf{External Validity} is related to the generalizability of our findings. Our study is based on Node.js applications that use npm. Hence our results may not generalize to applications written in other languages. However, the key concepts and design of our study can be applied on other package dependency networks. Although npm is a single case, examples from the past have shown that individual cases contribute to the building of a general empirical evidence software engineering~\cite{flyvbjerg2006five}. 

Our dataset contains 6,673 JavaScript applications that use npm packages. Our dataset might be considered small when it is compared to the whole population of JavaScript applications. However, our dataset is of high quality, since we filtered out applications that are immature and have less development history, by using the filtering criteria used by Kalliamvakou et al.~\cite{kalliamvakou2014promises}.


